ZeroSwap: Data-driven Optimal Market Making in DeFi

Automated Market Makers (AMMs) are major centers of matching liquidity supply and demand in Decentralized Finance. Their functioning relies primarily on the presence of liquidity providers (LPs) incentivized to invest their assets into a liquidity pool. However, the prices at which a pooled asset is traded is often more stale than the prices on centralized and more liquid exchanges. This leads to the LPs suffering losses to arbitrage. This problem is addressed by adapting market prices to trader behavior, captured via the classical market microstructure model of Glosten and Milgrom. In this paper, we propose the first optimal Bayesian and the first model-free data-driven algorithm to optimally track the external price of the asset. The notion of optimality that we use enforces a zero-profit condition on the prices of the market maker, hence the name ZeroSwap. This ensures that the market maker balances losses to informed traders with profits from noise traders. The key property of our approach is the ability to estimate the external market price without the need for price oracles or loss oracles. Our theoretical guarantees on the performance of both these algorithms, ensuring the stability and convergence of their price recommendations, are of independent interest in the theory of reinforcement learning. We empirically demonstrate the robustness of our algorithms to changing market conditions.

==> variable_trade_size.tex <==
% \subsection{Model}\label{sec:model_general}
%   The discussion so far concerns obtaining an efficient market maker for the case of a fixed trade size. We now modify our model to allow variable trade size and generalize the behaviour of traders. The rest of the model stays the same as described in \prettyref{sec:model}.
  
% \textbf{Trader behavior : }We assume traders see a noisy version of the external price in each time step, denoted by $p_{trad}^t$ and given by 
% \begin{align}
%     p_{trad}^t &= p_{ext}^t + \eta_t
% \end{align}
% where $\eta_t$ is i.i.d. noise sampled at each time step.

% \textbf{Trade actions :} The market maker publishes a \textit{demand curve}\cite{milionis2023myersonian} at each time step, denoted by $g_t(p)$. The trader performs a trade that brings the operating point of the demand curve to $p_{trad}^t$. Thus, the trader behaves as if it is performing arbitrage between a market with price $p_{trad}^t$ and the demand curve published.

% \textbf{Objective :} Our objective remains as before, but extended to the modified trader behaviour.
% \begin{align}
%     p^t &= E[p_{ext}^t|\mathcal{H}_{t-1}, p^t_{trad}]\ \ \ \ \forall p^t_{trad} \label{eq:gm_price_modified}
% \end{align}
% where $\mathcal{H}_{t-1} = \langle (p_{trad}^{\tau},g_{\tau}(.))\rangle_{\tau=0}^{t-1}$ is the history of trades and demand curves until time $t-1$.

% \color{red}
% show typical model parameter values for uniswap trading data?
% \color{black}

% \subsection{Bayesian Algorithm}

% In this section, we derive the optimal behavior in case we know the distribution of the noise $\eta_t$ through which the traders observe the external price.

% As mentioned in \prettyref{sec:model_general}, we make use of the general demand curve formulation for market makers, as explained in \cite{milionis2023myersonian}. Assume that the amount of asset in reserves at any price $p_0$ is $g_t(p_0)$, while the amount of numeraire is $-\int_0^{p_0} p dg_t(p)$. If price is constrained to be on discrete ticks of size $\delta$, then the numeraire amount becomes $-\sum_{k=0}^{p_0/\delta} k\delta (g_t(k\delta) - g_t((k-1)\delta))$. The function $g_t$ needs to be non-increasing for the AMM to be stable.

% Let $f_t$ be the belief of the AMM over prices at time $t$. Let $f_\eta$ be the distribution of noise through which the price is observed by the traders. Let $p_{trad}$ be the price that the trader observes. Then, the trader would make a trade with the AMM such that the marginal price of the asset just after the trade is $p_{trad}$. 

% In this case, the GM conditions can be written as
% \begin{align}
%     \frac{-\int_{p_0}^{p_{trad}^t} p dg_t(p)}{g_t(p_0)-g_t(p_{trad}^t)} &= \frac{\int_0^\infty pf_{\eta}(p_{trad}^t-p)f_t(p)dp}{\int_0^\infty f_{\eta}(p_{trad}^t-p)f_t(p)dp} 
% \end{align}
% Rearranging gives us 
% \begin{align}
%     g_t(p_{trad}^t) = x_0 + \frac{\int_{p_0}^{p_{trad}^t}pg'_t(p)dp}{\beta(p_{trad}^t)}
% \end{align}
% where $\beta_t(p_{trad}^t) = \frac{\int_0^\infty pf_{\eta}(p_{trad}^t-p)f_t(p)dp}{\int_0^\infty f_{\eta}(p_{trad}^t-p)f_t(p)dp} $, and the constant $x_0$ being the amount of asset in the AMM just before the trade, and $p_0$ is the solution to the fixed point equation $p=\beta(p)$. 

% The demand curve can also be said to obey the following differential equation in $p$
% \begin{align}
%     (\beta_t(p)g_t(p))' - pg'_t(p) - \beta_t'(p) x_0 = 0
% \end{align}
% with the constraints $g(p_0) = x_0$ where $p_0=\beta(p_0)$.


% After the trade, we update our beliefs as 
% \begin{align}
%     f_{t+1}(p) = \frac{f_{\eta}(p_{trad}^t-p)f_t(p)}{\int_0^\infty f_{\eta}(p_{trad}^t-p)f_t(p)dp} 
% \end{align}

% %Changing the curve as per the above equations also opens the door to adversarial exploitation?

% \textbf{Numerical implementation : }While implementing the equations above, we discretize the demand curve and the belief functions as vectors. At the end of the $t^{th}$ time step, we have the posterior vector $f_t(p)$ as our belief over the external price. The number of components of the vector are equal to the number of price ticks $N$ in our AMM. Therefore, $f_t,g_t\in \mathbb{R}^N$. We first calculate the $\beta_t-$ vector as follows
% \begin{align}
%     \beta_t(p) = \frac{\sum_{k=1}^N k\delta f_{\eta}(p-k\delta)f_t(k\delta)}{\sum_{k=1}^N f_{\eta}(p-k\delta)f_t(k\delta)} 
% \end{align}
% where $f_{\eta}$ is the noise distribution vector and $\delta$ is the tick size. 

% Next, we find the price $p_0$ such that
% \begin{align}
%     p_0=\beta_t(p_0) 
% \end{align}
% We now define our demand vector $g_t\in \mathbb{R}^N$
% and set $g_t(p_0) = x_0$.

% Next, we obtain the rest of the components of the $g-$vector by the following formula
% \begin{align}
% g_t(p)&=
% \begin{cases}
%         x_0 \ \ &\mathrm{if\ }p=p_0\\
%         x_0+\frac{\sum_{k=p_0/\delta+1}^{p/\delta} k\delta (g_t(k\delta) - g_t((k-1)\delta))}{\beta_t(p)} \ \ &\mathrm{if\ }p > p_0\\
%          x_0-\frac{\sum_{k=p/\delta}^{p_0/\delta-1} k\delta (g_t(k\delta) - g_t((k-1)\delta))}{\beta_t(p)} \ \ &\mathrm{if\ }p < p_0
%     \end{cases}
% \end{align}

% The vector $g_t$ is presented to the trader, and the trader chooses $p^{trad}_t$. Then, we update the posterior for the next time step as follows
% \begin{align}
%     f_{t+1}(p) = \frac{f_{\eta}(p^{trad}_t-p)f_t(p)}{\sum_{k=1}^N f_{\eta}(p^{trad}_t-k\delta)f_t(k\delta)} 
% \end{align}


% Empirically, we find the solution to be a single value $p_0$ with discontinuity, and the demand curve to be constant on the rest of $p\in [0,\infty)$. This implies a constant sum market maker with slope equal to $p_0$. Any market maker that has a slope of $p_0$ at reserve value $x_0$ and a positive curvature would thus collect a strictly positive expected profit.

% Implementing the Bayesian variable trade size market maker gives us better profit than in the case of a static market maker. This has been shown in \prettyref{fig:}. 

% \color{red}
% <figure showing simulation results for the above claim> 
% \color{black}

% It now remains to formulate a reward function that replicates this behaviour in the case when the underlying model is unknown. 

%  \color{red}

% \subsection{Data-driven algorithm for the general model}

% modified reward function and intuition

% algorithm used

% simulation results

% \subsection{Implementation}

% implementation on layer 2 platforms such as base, bold


% \color{black}
